Proximal Gradient Descent-Ascent: Variable Convergence under K{\L} Geometry

The gradient descent-ascent (GDA) algorithm has been widely applied to solve minimax optimization problems. In order to achieve convergent policy parameters for minimax optimization, it is important that GDA generates convergent variable sequences rather than convergent sequences of function values or gradient norms. However, the variable convergence of GDA has been proved only under convexity geometries, and there lacks understanding for general nonconvex minimax optimization. This paper fills such a gap by studying the convergence of a more general proximal-GDA for regularized nonconvex-strongly-concave minimax optimization. Specifically, we show that proximal-GDA admits a novel Lyapunov function, which monotonically decreases in the minimax optimization process and drives the variable sequence to a critical point. By leveraging this Lyapunov function and the K{\L} geometry that parameterizes the local geometries of general nonconvex functions, we formally establish the variable convergence of proximal-GDA to a critical point $x^*$, i.e., $x_t\to x^*, y_t\to y^*(x^*)$. Furthermore, over the full spectrum of the K{\L}-parameterized geometry, we show that proximal-GDA achieves different types of convergence rates ranging from sublinear convergence up to finite-step convergence, depending on the geometry associated with the K{\L} parameter. This is the first theoretical result on the variable convergence for nonconvex minimax optimization.

==> assumption1.tex <==
\section{Proof of the relationship among the statements in Assumption 1}\label{sec_assum1}

We will prove that in \Cref{assum: f}, the item 2 and the statement that $g$ is lower semi-continuous can be derived from the rest of \Cref{assum: f}. 
\begin{proof}
	\noindent Since the sub-level set $\{x: (\Phi+g)(x)\le\alpha\}$ is closed, $\Phi+g$ is lower semi-continuous. Without item 2 and any assumption on $g$, Lemma \Cref{prop_Phiystar} holds which implies continuity of $\Phi$, so $g$ is lower semi-continuous.  
	
	%\noindent If the sub-level set $A=\{x: (\Phi+g)(x)\le0 \}$ is empty, then 0 is a lower bound of $\Phi+g$. Hence, we focus on the case where $A$ is non-empty convex set.\\
	
	\noindent Suppose $\Phi+g$ is not bounded below, then there is a sequence $\{x_t\}_t$ such that $(\Phi+g)(x_t)\le -t$. Since $x_t\in A$ and $A$ is compact, $\{x_n\}$ has at one convergent subsequence $x_{n(t)}\overset{t}{\to} x^*$. Since $\Phi+g$ is lower semi-continuous, $\Phi(x^*)+g(x^*)\le \mathop{\lim\inf}_{n\to\infty} \Phi(x_{n(t)})+g(x_{n(t)})=-\infty$. However, since $\Phi$ is continuous and $g$ is proper, $\Phi(x^*), g(x^*)>-\infty$, is a contradiction. Hence, $\Phi+g$ is not bounded below, that is, the item 2 of \Cref{assum: f} holds
\end{proof}

==> introduction.tex <==
\section{Introduction}
A majority of machine learning applications are naturally formulated as nonconvex optimization due to the complex mechanism of the underlying model. Typical examples include training neural networks in deep learning \cite{Goodfellow2016}, low-rank matrix factorization \cite{RongGe2016,Bhojanapalli2016}, phase retrieval \cite{Candes2015,Zhang2017}, etc. In particular, these machine learning problems take the generic form
\begin{align*}
\min_{\xb\in \RR^d}~~f(\xb), \tag{P}
\end{align*}
where the objective function $f: \RR^d \to \RR$ is a differentiable and nonconvex function, and usually corresponds to the total loss over a set of data samples. 
Traditional first-order algorithms such as gradient descent can produce a solution $\bar{\xb}$ that satisfies the first-order stationary condition, i.e., $\nabla f (\bar{\xb}) = \zero$. However, such first-order stationary condition does not exclude the possibility of approaching a saddle point, which can be a highly suboptimal solution and therefore deteriorate the performance. 

Recently in the machine learning community, there has been an emerging interest in designing algorithms to scape saddle points in nonconvex optimization, and one popular algorithm is the cubic-regularized Newton's algorithm \cite{Nesterov2006,Agarwal2017,Yue2018}, which is also referred to as cubic regularization (CR) for simplicity. Such a second-order method exploits the Hessian information and produces a solution $\bar{\xb}$ for problem (P) that satisfies the second-order stationary condition, i.e., 
$$(\text{second-order stationary}):\quad \nabla f (\bar{\xb}) = \zero, ~\nabla^2 f(\bar{\xb}) \succeq \zero.$$
The second-order stationary condition ensures CR to escape saddle points wherever the corresponding Hessian matrix has a negative eigenvalue (i.e., strict saddle points \cite{Sun2015}). In particular, many nonconvex machine learning problems have been shown to exclude spurious local minima and have only strict saddle points other than global minima \cite{Baldi1989,Sun2017,RongGe2016,zhou2018}. In such a desirable case, CR is guaranteed to find the global minimum for these nonconvex problems. 
To be specific, given a proper parameter $M>0$, CR generates a variable sequence $\{ \xb_{k}\}_k$ via the following update rule
\begin{align}
	\text{(CR)}~ \xb_{k+1} \in \argmin_{\yb \in \RR^d} ~\inner{\yb - \xb_{k}}{\nabla f (\xb_{k})} + \frac{1}{2} (\yb - \xb_{k})^\ttop \nabla^2 f(\xb_{k})  (\yb - \xb_{k}) + \frac{M}{6} \|\yb - \xb_{k}\|^3. \label{eq: CR}
\end{align}
Intuitively, CR updates the variable by minimizing an approximation of the objective function at the current iterate. This approximation is essentially the third-order Taylor's expansion of the objective function. We note that computationally efficient solver has been proposed for solving the above cubic subproblem \cite{Agarwal2017}, and it was shown that the resulting computation complexity of CR to achieve a second-order stationary point serves as the state-of-the-art among existing algorithms that achieve the second-order stationary condition.
%is lower than that of gradient descent to achieve a first-order stationary point.

Several studies have explored the convergence of CR for nonconvex optimization. Specifically, the pioneering work \cite{Nesterov2006} first proposed the CR algorithm and showed that the variable sequence $\{\xb_{k} \}_k$ generated by CR has second-order stationary limit points and converges sub-linearly. Furthermore, the gradient norm along the iterates was shown to converge quadratically (i.e., super-linearly) given an initialization with positive definite Hessian. Moreover, the function value along the iterates was shown to converge super-linearly under a certain gradient dominance condition of the objective function. Recently, \cite{Yue2018} studied the asymptotic convergence rate of CR under the local error bound condition, and established the quadratic convergence of the distance between the variable and the solution set. 
Clearly, these results demonstrate that special geometrical properties (such as the gradient dominance condition and the local error bound) enable much faster convergence rate of CR towards a second-order stationary point. However, these special conditions may fail to hold for generic complex objectives involved in practical applications. Thus, it is desired to further understand the convergence behaviors of CR for optimizing nonconvex functions over a broader spectrum of geometrical conditions.

The Kurdyka-{\L}ojasiewicz (K{\L}) property (see \Cref{sec: pre} for details) \cite{Bolte2007,Bolte2014} serves as such a candidate. As described in \Cref{sec: pre}, the \KL property captures a broad spectrum of the local geometries that a nonconvex function can have and is parameterized by a parameter $\theta$ that changes over its allowable range.  In fact, the \KL property has been shown to hold ubiquitously for most practical functions (see \Cref{sec: pre} for a list of examples). 
The \KL property has been exploited extensively to analyze the convergence rate of various {\em first-order} algorithms for nonconvex optimization, e.g., gradient method \cite{Attouch2009,Li2017}, alternating minimization \cite{Bolte2014} and distributed gradient methods \cite{Zhou2016}.
But it has not been exploited to establish the {\em convergence rate} of second-order algorithms towards second-order stationary points.  
In this paper, we exploit the \KL property of the objective function to provide a comprehensive study of the convergence rate of CR for nonconvex optimization. We anticipate our study to substantially advance the existing understanding of the convergence of CR to a much broader range of nonconvex functions. We summarize our contributions as follows.
\vspace{-5pt}
\subsection{Our Contributions}
\vspace{-5pt}
We characterize the convergence rate of CR locally towards second-stationary points for nonconvex optimization under the \KL property of the objective function. Our results also compare and contrast the different order-level of guarantees that \KL yields between the first and second-order algorithms.
Also, our analysis characterizes the convergence property for a range of \KL parameter $\theta$,  which requires the development of different recursive inequalities for various cases.

\textbf{Gradient norm \& least eigenvalue of Hessian:}
We characterize the asymptotic convergence rates of the sequence of gradient norm $\{\|\nabla f(\xb_{k})\| \}_k$ and the sequence of the least eigenvalue of Hessian $\{\lambda_{\min} (\nabla^2 f(\xb_{k}))\}_k$ generated by CR. We show that CR meets the second-order stationary condition at a (super)-linear rate in the parameter range $\theta \in [\frac{1}{3}, 1]$ for the \KL property, while the convergence rates become sub-linearly in the parameter range $\theta \in (0, \frac{1}{3})$ for the \KL property.

\textbf{Function value gap \& variable distance:} 
We characterize the asymptotic convergence rates of the function value sequence $\{f(\xb_{k})\}_k$ and the variable sequence $\{\xb_{k}\}_k$ to the function value and the variable of a second-order stationary point, respectively. The obtained convergence rates range from sub-linearly to super-linearly depending on the parameter $\theta$ associated with the \KL property. Our convergence results generalize the existing ones established in \cite{Nesterov2006} corresponding to special cases of $\theta$ to the full range of $\theta$. Furthermore, these types of convergence rates for CR are orderwise faster than the corresponding convergence rates of the first-order gradient descent algorithm in various regimes of the \KL parameter $\theta$ (see \Cref{table: 1} and \Cref{table: 2}  for the comparisons). 

Based on the \KL property, we establish a generalized local error bound condition (referred to as the \KL error bound). The \KL error bound further leads to characterization of the convergence rate of distance between the variable and the solution set, which ranges from sub-linearly to super-linearly depending on the parameter $\theta$ associated with the \KL property.
This result generalizes the existing one established in \cite{Yue2018} corresponding to a special case of $\theta$ to the full range of $\theta$. 


\vspace{-5pt}
\subsection{Related Work}
\vspace{-5pt}
\textbf{Cubic regularization:} CR algorithm was first proposed in \cite{Nesterov2006}, in which the authors analyzed the convergence of CR to second-order stationary points for nonconvex optimization. In \cite{Nesterov2008}, the authors established the sub-linear convergence of CR for solving convex smooth problems, and they further proposed an accelerated version of CR with improved sub-linear convergence. Recently, \cite{Yue2018} studied the asymptotic convergence properties of CR under the error bound condition, and established the quadratic convergence of the iterates. Several other works proposed different methods to solve the cubic subproblem of CR, e.g., \cite{Agarwal2017,Carmon2016,Cartis2011a}.


\textbf{Inexact-cubic regularization:} 
Another line of work aimed at improving the computation efficiency of CR by solving the cubic subproblem with inexact gradient and Hessian information. In particular, \cite{Saeed2017,Jin2017} proposed an inexact CR for solving convex problem and nonconvex problems, respectively. Also, \cite{Cartis2011b} proposed an adaptive inexact CR for nonconvex optimization, whereas \cite{Jiang2017} further studied the accelerated version for convex optimization. Several studies explored subsampling schemes to implement inexact CR algorithms, e.g., \cite{kohler2017,Xu2017,Zhou2018,Wang2018}. 


\textbf{\KL property:} The \KL property was first established in \cite{Bolte2007}, and was then widely applied to characterize the asymptotic convergence behavior for various first-order algorithms for nonconvex optimization \cite{Attouch2009,Li2017,Bolte2014,Zhou2016,Zhou_2017a}. The \KL property was also exploited to study the convergence of second-order algorithms such as generalized Newton's method \cite{Frankel2015} and the trust region method \cite{Noll2013}. However, these studies did not characterize the convergence rate and the studied methods cannot guarantee to converge to second-order stationary points, whereas this paper provides this type of results.

\textbf{First-order algorithms that escape saddle points:} Many first-order algorithms are proved to achieve second-order stationary points for nonconvex optimization. For example, online stochastic gradient descent \cite{Ge2015}, perturbed gradient descent \cite{Jin2017}, gradient descent with negative curvature \cite{Carmon2016,Liu2017} and other stochastic algorithms \cite{Zhu2017}.


